Max Weight Independent Set in sparse graphs with no long claws

We revisit the recent polynomial-time algorithm for the MAX WEIGHT INDEPENDENT SET (MWIS) problem in bounded-degree graphs that do not contain a fixed graph whose every component is a subdivided claw as an induced subgraph [Abrishami, Dibek, Chudnovsky, Rz\k{a}\.zewski, SODA 2022]. First, we show that with an arguably simpler approach we can obtain a faster algorithm with running time $n^{\mathcal{O}(\Delta^2)}$, where $n$ is the number of vertices of the instance and $\Delta$ is the maximum degree. Then we combine our technique with known results concerning tree decompositions and provide a polynomial-time algorithm for MWIS in graphs excluding a fixed graph whose every component is a subdivided claw as an induced subgraph, and a fixed biclique as a subgraph.

==> problem.tex <==
Instead of solving \MWIS, we will actually solve a more general problem, defined as follows.


\problemTask{\probname}{A graph $G$, a weight function $\wei : V(G) \to \N$, a set $T \subseteq V(G)$}{For each $S \subseteq T$, compute a maximum-weight independent set $I_S$ in $G$ with $I \cap T = S$}

Clearly \MWIS can be solved by solving an instance of \probname with $T = \emptyset$ and returning the only computed set, i.e., $I_\emptyset$.
